Polyhedral Aspects of Feedback Vertex Set and Pseudoforest Deletion Set

We consider the feedback vertex set problem in undirected graphs (FVS). The input to FVS is an undirected graph $G=(V,E)$ with non-negative vertex costs. The goal is to find a minimum cost subset of vertices $S \subseteq V$ such that $G-S$ is acyclic. FVS is a well-known NP-hard problem and does not admit a $(2-\epsilon)$-approximation for any fixed $\epsilon > 0$ assuming the Unique Games Conjecture. There are combinatorial $2$-approximation algorithms and also primal-dual based $2$-approximations. Despite the existence of these algorithms for several decades, there is no known polynomial-time solvable LP relaxation for FVS with a provable integrality gap of at most $2$. More recent work (Chekuri and Madan, SODA '16) developed a polynomial-sized LP relaxation for a more general problem, namely Subset FVS, and showed that its integrality gap is at most $13$ for Subset FVS, and hence also for FVS. Motivated by this gap in our knowledge, we undertake a polyhedral study of FVS and related problems. In this work, we formulate new integer linear programs (ILPs) for FVS whose LP-relaxation can be solved in polynomial time, and whose integrality gap is at most $2$. The new insights in this process also enable us to prove that the formulation in (Chekuri and Madan, SODA '16) has an integrality gap of at most $2$ for FVS. Our results for FVS are inspired by new formulations and polyhedral results for the closely-related pseudoforest deletion set problem (PFDS). Our formulations for PFDS are in turn inspired by a connection to the densest subgraph problem. We also conjecture an extreme point property for a LP-relaxation for FVS, and give evidence for the conjecture via a corresponding result for PFDS.

==> results.tex <==
\subsection{Results}
%We present formal statements of our results in this section. 
We recall that our main goal is to formulate an integer linear program
(ILP) for FVS whose LP-relaxation has integrality gap at most $2$. As
our first result, we show how to achieve this goal for PFDS by giving
a new ILP formulation. We will subsequently use the properties of our
new ILP formulation for PFDS to achieve the goal for FVS.

Our new ILP for PFDS is based on Charikar's LP for the densest
subgraph problem (DSG) \cite{charikar_greedy_2000}. In DSG, the input is
an undirected graph $G=(V,E)$ and the goal is to find an induced subgraph $G[S]$ of
maximum density where the density of $S \subseteq V$ is defined
as $\frac{|E(S)|}{|S|}$. We define the density of $G$ to be $\max\{|E[S]|/|S|: \emptyset \ne S\subseteq V\}$. We note that a graph is a pseudoforest if and only if
its density is at most one. Thus, PFDS can equivalently be phrased as
the problem of finding a minimum cost subset of vertices to delete so
that the remaining graph has density at most one.  Charikar formulated
an LP to compute the density of a graph. The dual of Charikar's LP can
be interpreted as a fractional orientation problem.  Using that dual,
we obtain an ILP for PFDS. Our ILP for PFDS is based on the following
polyhedron that will be denoted as the orientation polyhedron:

%have the following LP-relaxation for PFDS for a graph $G$: $\min \{\sum_{u\in V}c_u x_u: \exists\ z_e^u\ \forall e\in \delta(u),\ u\in V\text{ such that }(x, z)\in \orientationpolyhedron(G)\}$, where

\begin{align*}
\orientationpolyhedron(G):=
\left\{ (x,y): \begin{array}{l}
x_u + x_v+ y_{e,u} + y_{e,v} \ge 1\ \forall e\in E: e=uv\\
x_u + \sum_{e\in \delta(u)} y_{e,u} \le 1\ \forall u \in V\\
x_u \ge 0\ \forall u\in V\\
y_{e,u} \ge 0\ \forall e\in \delta(u), u\in V.
  \end{array}\right\}.
\end{align*}
We will denote the projection of $\orientationpolyhedron(G)$ to the $x$ variables by $\projectedorientationpolyhedron(G)$. 

\begin{restatable}{theorem}{lemmaOrientationFormulation}
\label{lemma:orientation-formulation}
The following are integer linear programming formulations for PFDS for a graph $G=(V, E)$ with non-negative costs $c: V\rightarrow \R_{\ge 0}$:
\begin{align}
\min &\left\{\sum \nolimits_{u\in V}c_u x_u: x\in \projectedorientationpolyhedron(G)\cap \Z^V\right\} \text{ and} \tag{PFDS-IP: orient} \label{PFDS-IP:orient}\\
\min &\left\{\sum \nolimits_{u\in V}c_u x_u: x\in \projectedorientationpolyhedron(G)\cap \twopseudotreecoverpolyhedron(G)\cap \Z^V\right\}. \tag{PFDS-IP: orient-and-2PT-cover} \label{PFDS-IP:Orient-and-2PT-cover} 
\end{align}
Moreover, we have the following properties:
\begin{enumerate}
\item $\projectedorientationpolyhedron(G)\subseteq \weakdensitypolyhedron(G)$ for every graph $G$ and there exist graphs $G$ for which $\projectedorientationpolyhedron(G)\subsetneq \weakdensitypolyhedron(G)$. 

\item The integrality gap of the following LP-relaxation is at most $2$:
    \begin{align}
    \min &\left\{\sum \nolimits_{u\in V}c_u x_u: x\in \projectedorientationpolyhedron(G)\cap \twopseudotreecoverpolyhedron(G) \right\}. \tag{PFDS-LP: orient-and-2PT-cover} \label{PFDS-LP:Orient-and-2PT-cover} 
    \end{align}

\item There exists a polynomial-time separation oracle for the family of $2$-pseudotree cover constraints. 
\end{enumerate}
\end{restatable}

%The integrality gap of (\ref{PFDS-LP: Orient}) is at least $3$ as illustrated by the example in \Cref{fig:butterfly-orientation-integrality-gap}. 
We note that the upper bound of $2$ on the integrality gap of
(\ref{PFDS-LP:Orient-and-2PT-cover}) mentioned in
\Cref{lemma:orientation-formulation} is tight as shown in Figure \ref{fig:orientation-2PT-cover-integrality-gap-instance}. 
As a consequence of \Cref{lemma:orientation-formulation}, we
immediately obtain an integer linear program for PFDS
whose LP-relaxation is solvable in polynomial time and has integrality gap at most $2$ --- namely
(\ref{PFDS-IP:Orient-and-2PT-cover}). We also bound the integrality
gap of the LP-relaxation of (\ref{PFDS-IP:orient}), but this will be
based on extreme point properties and will be discussed later in this
section.

\begin{figure}[H]
    \centering
\includegraphics[width=0.4\textwidth]{images/Orientation-2PTCover-Integrality-Gap-Instance.png}
    \caption{An example showing that the integrality gap of (\ref{PFDS-LP:Orient-and-2PT-cover}) tends to $2$ as $n$ tends to infinity. Consider the graph $G=(V, E)$ as shown above (where $K_n$ denotes the complete graph on $n$ vertices) with cost of every vertex $a\in V-\{u, v, w\}$ being $1$ and costs of vertices $u, v, w$ being infinite. The optimum value of (\ref{PFDS-IP:Orient-and-2PT-cover}) is $n-1$. The optimum value of (\ref{PFDS-LP:Orient-and-2PT-cover}) is at most $n/2$: the solution $x_a = 1/2$ for every vertex $a\in V-\{u, v, w\}$, $x_u = x_v = x_w = 0$, $y_{e, a}=0$ for all edges $e=ab$ where $a, b\in V-\{u, v, w\}$, $y_{uv, v}=y_{vw, w}=y_{wu,u}=1$, $y_{uv, u} = y_{vw, v} = y_{wu, w} = 0$, and $y_{ua,a}=1/2$, $y_{ua, u} = 0$ for every $a\in V-\{u, v,w\}$ is feasible for (\ref{PFDS-LP:Orient-and-2PT-cover}) and has cost $n/2$.}
    \label{fig:orientation-2PT-cover-integrality-gap-instance}
\end{figure}
%\knote{Can conclusion 1 of the above theorem be proven via extreme point property (for $\weakdensitypolyhedron(G)\cap \twopseudotreecoverpolyhedron(G)$)? Or is there an example similar to \Cref{fig:butterfly-orientation-integrality-gap}?}

Next, we focus on formulating an ILP for FVS whose LP-relaxation has
integrality gap at most $2$ and is polynomial-time solvable. In order
to achieve this goal, we formulate an intermediate ILP for FVS whose
LP-relaxation has integrality gap at most $2$, but it is unclear if
this LP-relaxation is polynomial-time solvable.  We will later
formulate a \emph{polynomial-sized} ILP for FVS whose LP-relaxation is
at least as strong as that of the intermediate ILP, thereby achieving
our goal.

Our intermediate ILP is based on weak density constraints and the following polyhedron that will be denoted as the cycle cover polyhedron: 
\begin{align}
\cyclecoverpolyhedron(G)&:=\left\{x\in \R^V_{\ge 0}: \sum \nolimits_{u\in U}x_u \ge 1 \ \forall U\subseteq V \text{ such that $G[U]$ is a cycle}\right\}. \label{eqn:cycle-cover}
\end{align}
We will denote the constraints describing the cycle cover polyhedron as cycle cover constraints. 
%We note that weak density constraints are valid for PFDS and consequently, are also valid for FVS. Cycle cover constraints are also valid for FVS. The validity of these two families of constraints for FVS motivates the following natural ILP for FVS: $\min\{\sum_{u\in V}c_u x_u: x\in \weakdensitypolyhedron(G)\cap \cyclecoverpolyhedron(G)\cap \Z^V\}$. 
%We will focus on its LP-relaxation and bound its integrality gap. 
%\begin{align}
%\min\left\{\sum_{u\in V} c_u x_u: x\in \weakdensitypolyhedron(G)\cap \cyclecoverpolyhedron(G)\right\}. \tag{WD-CC-LP}\label{LP:weak-density-cycle-cover}
%\end{align}
%Although we do not have a polynomial-time algorithm to solve its LP-relaxation, we will later see that it is helpful to understand its integrality gap. We prove that its integrality gap is at most $2$. 
%It is easy to see that the integrality gap of (\ref{LP:weak-density-cycle-cover}) is at most $4$: By \Cref{cor:thm:integrality-gap-3-orientation}, there exists a solution $S\subseteq V$ for PFDS such that $\sum_{u\in S}c_u\le 3 \sum_{u\in V}c_u x_u$; for each component in $G-S$ that contains a cycle, add the least cost vertex of the cycle to a set $T$; we note that $\sum_{u\in T}c_u\le \sum_{u\in V}c_u x_u$. Now, the set $S\cup T$ is a  feedback vertex set of $G$ with $\sum_{u\in S\cup T}c_u\le 4\sum_{u\in V}c_ux_u$ and consequently, the integrality gap of (\ref{LP:weak-density-cycle-cover}) is at most $4$. Our next result improves on this integrality gap.

\begin{theorem}\label{thm:integrality-gap-wd+cycle-cover}
The following is an integer linear programming formulation for FVS for a graph $G=(V, E)$ with non-negative costs $c: V\rightarrow \R_{\ge 0}$: 
\begin{align}
\min\left\{\sum \nolimits_{u\in V}c_u x_u: x\in \weakdensitypolyhedron(G)\cap \cyclecoverpolyhedron(G)\cap \Z^V\right\}. \tag{FVS-IP: WD-and-cycle-cover} \label{FVS-IP: WD-and-cycle-cover}
\end{align}
Moreover, we have the following properties: 
\begin{enumerate}
    \item The integrality gap of the following LP-relaxation is at most $2$: 
\begin{align*}
\min\left\{\sum \nolimits_{u\in V} c_u x_u: x\in \weakdensitypolyhedron(G)\cap \cyclecoverpolyhedron(G)\right\}. \tag{FVS-LP: WD-and-cycle-cover}
\label{FVS-LP:weak-density-cycle-cover}
\end{align*}
    \item There exists a polynomial-sized formulation for $\cyclecoverpolyhedron(G)$.  
\end{enumerate}
\end{theorem}
%It is tempting to prove \Cref{thm:integrality-gap-wd+cycle-cover} via an extreme point structural result in the spirit of \Cref{thm:weak-density-extreme-point}: if we could show that every extreme point had a co-ordinate with value at least $1/2$, then we would have an alternative proof of \Cref{thm:integrality-gap-wd+cycle-cover} via the  iterative rounding technique. However, the example given in \Cref{fig:K4-WD-CC-integrality-gap} shows that the former statement is false. Instead of the extreme point based proof technique, our proof of \Cref{thm:integrality-gap-wd+cycle-cover} is via the primal-dual algorithm and is a modification of a primal-dual algorithm for FVS using strong density constraints given by Chudak, Goemans, Hochbaum, and Williamson \cite{CHUDAK1998111}. 
\Cref{thm:integrality-gap-wd+cycle-cover} shows that (\ref{FVS-IP: WD-and-cycle-cover}) is an ILP for FVS whose LP-relaxation (\ref{FVS-LP:weak-density-cycle-cover}) has integrality gap at most $2$. However, we do not have a polynomial-time algorithm to solve the LP-relaxation (\ref{FVS-LP:weak-density-cycle-cover}) --- this is because, we do not have a polynomial-time separation oracle for the family of weak density constraints (although we do have a polynomial-time separation oracle for the family of cycle cover constraints). 
We will use \Cref{lemma:orientation-formulation} in conjunction with \Cref{thm:integrality-gap-wd+cycle-cover} to prove the following result: 
%We will use \Cref{lemma:orientation-formulation} to conclude that the orientation polyhedron is at least as strong as the weak density polyhedron while observing that its constraints are still valid for FVS thereby leading to the following result: 
%To resolve this, it suffices to give a \emph{polynomial-sized} ILP formulation for FVS whose constraints are at least as strong as weak density constraints. We will use \Cref{lemma:orientation-formulation} to conclude that this is achieved by the orientation polyhedron. Consequently, we have the following result: 

\begin{theorem}\label{thm:poly-sized-LP-with-integrality-gap-atmost-2-for-FVS} 
There exists a polynomial-sized integer linear programming formulation for FVS whose LP-relaxation has integrality gap at most $2$. 
\end{theorem}
We prove \Cref{thm:poly-sized-LP-with-integrality-gap-atmost-2-for-FVS} by showing three different polynomial-sized integer linear programs for FVS all of whose LP-relaxations have integrality gap at most $2$:
\begin{enumerate}
\item The first formulation is 
\begin{align}
    \min\left\{\sum \nolimits_{u\in V}c_u x_u: x\in \projectedorientationpolyhedron(G)\cap \cyclecoverpolyhedron(G)\cap \Z^V\right\}. \tag{FVS-IP: orient-and-cycle-cover} \label{FVS-IP: orient-and-cycle-cover}
\end{align}
%$\min\{\sum_{u\in V}c_u x_u: x\in \projectedorientationpolyhedron(G)\cap \cyclecoverpolyhedron(G)\cap \Z^V\}$. 
By \Cref{lemma:orientation-formulation}, we have that  $\projectedorientationpolyhedron(G)\subseteq \weakdensitypolyhedron(G)$. As a consequence of \Cref{thm:integrality-gap-wd+cycle-cover}, the integrality gap of the following LP-relaxation is also at most $2$: 
\begin{align}
    \min\left\{\sum \nolimits_{u\in V}c_u x_u: x\in \projectedorientationpolyhedron(G)\cap \cyclecoverpolyhedron(G)\right\}.  \tag{FVS-LP: orient-and-cycle-cover} \label{FVS-LP: orient-and-cycle-cover}
\end{align}
%$\min\{\sum_{u\in V}c_u x_u: x\in \projectedorientationpolyhedron(G)\cap \cyclecoverpolyhedron(G)\}$ 
Both $\projectedorientationpolyhedron(G)$ and $\cyclecoverpolyhedron(G)$ admit a polynomial-sized description, and thus, we have a polynomial-sized ILP for FVS whose LP-relaxation has integrality gap at most $2$.

\item The second formulation is the Chekuri-Madan formulation who, as
  we remarked earlier, formulated an ILP for Subset-FVS and showed
  that the integrality gap of its LP-relaxation is at most $13$
  \cite{chekuri-madan16}. We show that
  their LP-relaxation specialized for FVS has integrality gap at most
  $2$ by proving that it is at least as strong as
%the LP-relaxation of our first formulation, i.e., 
  (\ref{FVS-LP: orient-and-cycle-cover}). Our result gives additional impetus
  to improving the integrality gap of the LP-relaxation for Subset-FVS. 

\item Our third formulation to prove \Cref{thm:poly-sized-LP-with-integrality-gap-atmost-2-for-FVS} is based on the orientation perspective, but without cycle cover constraints (as opposed to our first formulation). Here, we give an orientation based ILP formulation whose associated polyhedron is contained in the strong density polyhedron. Since the integrality gap of (\ref{FVS-LP: SD}) is at most $2$ (as shown by Chudak, Goemans, Hochbaum, and Williamson \cite{CHUDAK1998111}), the integrality gap of our third formulation is also at most $2$.   
\end{enumerate}
%\knote{Would be good to compare the three formulations relative to each other---is one stronger than the other or are they equivalent? Also, need to clarify that weak density constraints are weaker than orientation constraints - use Stefan's example from email.}
We emphasize that the proof of the integrality gap of the
LP-relaxation of all three of our ILPs rely on the integrality gap
bound of (\ref{FVS-LP:weak-density-cycle-cover}) or (\ref{FVS-LP:
  SD}). It would be interesting to have a direct proof: in particular,
it would be useful to design a primal rounding algorithm (for arbitrary
LP-optimum solutions or for extreme point LP-optimum solutions) that
yields a $2$-approximate solution.

\paragraph{Extreme point properties.} 
Motivated by \Cref{conj:strong-density-extreme-point} and the goal of
designing primal rounding algorithms for the LP relaxations for FVS,
we investigate extreme point properties of the weak density polyhedron
and the orientation polyhedron. Although we were unable to resolve
\Cref{conj:strong-density-extreme-point} for the strong density
polyhedron, we were able to prove an extreme point property for the
weak density polyhedron.

\begin{restatable}{theorem}{thmWeakDensityExtremePoint}
%\begin{theorem}
\label{thm:weak-density-extreme-point}
Let $G=(V, E)$ be a graph that is not a pseudoforest. For every extreme point $x$ of the polyhedron $\weakdensitypolyhedron(G)$, there exists a vertex $u \in V$ such that $x_u\geq 1/3$.
%\end{theorem}
\end{restatable}
Our proof of \Cref{thm:weak-density-extreme-point} is based on a
conditional supermodularity property---if all coordinates are small,
then the weak density constraints have a supermodular property; we use this
supermodular property to show the existence of a
structured basis for the extreme point which is subsequently used to arrive at a contradiction. To the best of authors' knowledge, the conditional
supermodularity property based proof has not previously appeared in the
literature on iterated rounding, and might be of independent interest.
\Cref{thm:weak-density-extreme-point} leads to the following
corollary.

%shows that the integrality gap of the weak density constraints based LP-relaxation for PFDS, namely $\min\{\sum_{u\in V}c_u x_u: x\in \weakdensitypolyhedron(G)\}$, is at most $3$. 

\iffalse
leads to an iterative-rounding based $3$-approximation algorithm for PFDS by repeatedly applying the following two steps until the graph $G$ is a pseudoforest:
(1) Compute an extreme point optimum solution $x$ of $\min\{\sum_{u\in V}c_u x_u: x\in P(G)$. 
(2) By \Cref{thm:weak-density-extreme-point}, there exists a vertex $u\in V$ such that $x_u \geq 1/3$; include the vertex $u$ in the solution and remove it from the graph $G$. The fact that this algorithm is a $3$-approximation also implies that the integrality gap of the weak-density constraints based LP-relaxation for PFDS, namely $\min\{\sum_{u\in V}c_u x_u: x\in \weakdensitypolyhedron(G)\}$, is at most $3$. 
\fi

\begin{thmcorollary}\label{cor:thm:integrality-gap-3-WD-PFD}
The integrality gap of the following LP-relaxation of (\ref{PFDS-IP: WD}) is at most $3$: 
\begin{align}
    \min\left\{\sum \nolimits_{u\in V}c_u x_u: x\in \weakdensitypolyhedron(G)\right\}. \tag{PFDS-LP: WD} \label{PFDS-LP: WD}
\end{align}
%The integrality gap of the LP-relaxation for PFDS given by $\min\{\sum_{u\in V}c_u x_u: x\in \weakdensitypolyhedron(G)\}$ is at most $3$.
\end{thmcorollary}
\Cref{cor:thm:integrality-gap-3-WD-PFD} can be seen to follow from \Cref{thm:weak-density-extreme-point} by the iterative rounding technique, where we repeatedly apply the following two steps until the graph $G$ is a pseudoforest: 
(1) Compute an extreme point optimum solution $x$ of (\ref{PFDS-LP: WD}). 
(2) By \Cref{thm:weak-density-extreme-point}, there exists a vertex $u\in V$ such that $x_u \geq 1/3$; include the vertex $u$ in the solution and remove it from the graph $G$. The approximation factor of the solution constructed by this procedure relative to the starting extreme point optimum solution to the LP is at most $3$.

The example given in \Cref{fig:butterfly-WD-integrality-gap} shows that the $(1/3)$-bound in \Cref{thm:weak-density-extreme-point} and  the integrality gap of $3$ mentioned in \Cref{cor:thm:integrality-gap-3-WD-PFD} are both tight. 
\input{images/K4-butterfly-examples}


 
We emphasize that the extreme point result given in \Cref{thm:weak-density-extreme-point} and the integrality gap result mentioned in Corollary \ref{cor:thm:integrality-gap-3-WD-PFD} are interesting only from a polyhedral viewpoint currently, and are not of help from the perspective of algorithm design. This is because, implementing the above-mentioned iterative rounding procedure requires us to solve the LP-relaxation (\ref{PFDS-LP: WD}) in polynomial time, but we do not know how to do this yet. 
%Although \Cref{cor:thm:integrality-gap-3-WD-PFD} shows that the integrality gap of the weak density constraints based LP-relaxation for PFDS, namely $\min\{\sum_{u\in V}c_u x_u: x\in \weakdensitypolyhedron(G)\}$ is at most $3$, we still do not know if this LP is solvable in polynomial time. 

We next show that although $\projectedorientationpolyhedron(G)$ is a subset of $\weakdensitypolyhedron(G)$ (as shown in \Cref{lemma:orientation-formulation}), the extreme point result for $\weakdensitypolyhedron(G)$ given in \Cref{thm:weak-density-extreme-point} still holds for $\projectedorientationpolyhedron(G)$. We will say that an extreme point of a polyhedron is \emph{minimal} if for each variable, reducing the value of that variable by any $\epsilon>0$ while keeping the rest of the variables unchanged results in a point that is outside the polyhedron. We note that extreme points of a polyhedron along non-negative objective directions will be minimal. 

\begin{restatable}{theorem}{thmOrientationPolyhedronExtremePoint}
%\begin{theorem}
\label{thm:orientation-polyhedron-extreme-point}
Let $G=(V, E)$ be a graph that is not a pseudoforest. For every minimal extreme point $(x,y)$ of the polyhedron $\orientationpolyhedron(G)$, there exists a vertex $u\in V$ such that $x_u\ge 1/3$. 
%\end{theorem}
\end{restatable}

\Cref{thm:orientation-polyhedron-extreme-point} leads to the following corollary (similar to \Cref{cor:thm:integrality-gap-3-WD-PFD} that follows from \Cref{thm:weak-density-extreme-point}): 
%it shows that the integrality gap of the orientation based LP-relaxation for PFDS, namely $\min \left\{\sum_{u\in V}c_u x_u: x\in \projectedorientationpolyhedron(G)\right\}$, is at most $3$. 

\begin{thmcorollary}\label{cor:thm:integrality-gap-3-orientation}
The integrality gap of the following LP-relaxation of (\ref{PFDS-IP:orient}) is at most $3$: 
\begin{align}
    \min\left\{\sum \nolimits_{u\in V}c_u x_u: x\in \projectedorientationpolyhedron(G)\right\} \tag{PFDS-LP: orient} \label{PFDS-LP:orient}
\end{align}
Moreover, given an extreme point optimum solution $x$ for the LP, there exists a polynomial time algorithm to obtain an integral feasible solution $x'$ for the LP-relaxation such that $\sum_{u\in V}c_u x'_u \le 3 \sum_{u\in V}c_u x_u$. 
\end{thmcorollary}

\Cref{cor:thm:integrality-gap-3-orientation} can be seen to follow from \Cref{thm:orientation-polyhedron-extreme-point} by the iterative rounding technique, where we repeatedly apply the following two steps until the graph $G$ is a pseudoforest: (1) Compute an extreme point optimum solution $x$ of $\min\left\{\sum_{u\in V}c_u x_u: x\in \projectedorientationpolyhedron(G)\right\}$. (2) By \Cref{thm:orientation-polyhedron-extreme-point}, there exists a vertex $u\in V$ such that $x_u\ge 1/3$; include the vertex $u$ in the solution and remove it from the graph $G$. The approximation factor of this procedure is $3$. In contrast to the weak density constraints based LP, namely (\ref{PFDS-LP: WD}), we can solve the orientation based LP, namely (\ref{PFDS-LP:orient}), in polynomial time. 


The example given in \Cref{fig:butterfly-orientation-integrality-gap} shows that the $(1/3)$-factor in \Cref{thm:orientation-polyhedron-extreme-point} 
%\knote{Adjust the caption to say `a minimal extreme point'. Do the values for $y$ in the current figure form a minimal extreme point? If not, then find such a $y$.} 
and the integrality gap of $3$ mentioned in \Cref{cor:thm:integrality-gap-3-orientation} are both tight. 
%\Cref{cor:thm:integrality-gap-3-orientation} implies that the ILP $\min\{\sum_{u\in V}c_u x_u: x\in \projectedorientationpolyhedron(G)\cap \Z^V\}$ for PFDS has the property that its LP-relaxation is polynomial-sized (and hence, polynomial-time solvable) and has integrality gap at most $3$. 

\input{images/oriented-butterfly-example.tex}

\begin{remark}
In the spirit of using iterative rounding to bound the integrality gap (e.g., \Cref{thm:weak-density-extreme-point} that leads to \Cref{cor:thm:integrality-gap-3-WD-PFD} and \Cref{thm:orientation-polyhedron-extreme-point} that leads to \Cref{cor:thm:integrality-gap-3-orientation}), it is tempting to bound the integrality gap of (\ref{FVS-LP:weak-density-cycle-cover}) by proving an extreme point result. In particular, if we could show that every extreme point optimum of (\ref{FVS-LP:weak-density-cycle-cover}) had a coordinate with value at least $1/2$, then we would have an alternative proof of the integrality gap bound mentioned in \Cref{thm:integrality-gap-wd+cycle-cover} via the  iterative rounding technique. However, the example given in \Cref{fig:K4-WD-CC-integrality-gap} shows that there exists an extreme point optimum of (\ref{FVS-LP:weak-density-cycle-cover}) all of whose coordinates have value at most $1/3$. 
\end{remark} 

\paragraph{Organization.} In Section \ref{sec:orientatin-polytope}, we prove properties of the orientation polyhedron and show \Cref{lemma:orientation-formulation}. 
In Section \ref{sec:weak-density-cycle-cover}, we prove properties of the weak density polyhedron, show that the cycle cover polyhedron admits a polynomial-sized formulation, and show \Cref{thm:integrality-gap-wd+cycle-cover}. 
In Section \ref{sec:poly-sized-lp-relaxation-with-gap-atmost-two-for-fvs}, we show three different polynomial-sized ILPs for FVS whose LP-relaxation has integrality gap at most $2$, thereby proving \Cref{thm:poly-sized-LP-with-integrality-gap-atmost-2-for-FVS}. In Sections \ref{sec:extreme-point-weak-density} and \ref{sec:orientation-polytope-extreme-point}, we prove extreme point properties of the weak density polyhedron and the orientation polyhedron and show \Cref{thm:weak-density-extreme-point} and \Cref{thm:orientation-polyhedron-extreme-point} respectively. 
